Evidence of spin-orbital angular momentum interactions in relativistic heavy-ion collisions

The first evidence of spin alignment of vector mesons ($K^{*0}$ and $\phi$) in heavy-ion collisions at the Large Hadron Collider (LHC) is reported. The spin density matrix element $\rho_{00}$ is measured at midrapidity ($|y| <$ 0.5) in Pb-Pb collisions at a center-of-mass energy ($\sqrt{s_{\rm NN}}$) of 2.76 TeV with the ALICE detector. $\rho_{00}$ values are found to be less than 1/3 (1/3 implies no spin alignment) at low transverse momentum ($p_{\rm T} <$ 2 GeV/$c$) for $K^{*0}$ and $\phi$ at a level of 3$\sigma$ and 2$\sigma$, respectively. No significant spin alignment is observed for the $K^0_S$ meson (spin = 0) in Pb-Pb collisions and for the vector mesons in $pp$ collisions. The measured spin alignment is unexpectedly large but qualitatively consistent with the expectation from models which attribute it to a polarization of quarks in the presence of angular momentum in heavy-ion collisions and a subsequent hadronization by the process of recombination.

==> fa_2019-10-13.tex <==
% Version: 2019-10-13

The ALICE Collaboration would like to thank all its engineers and technicians for their invaluable contributions to the construction of the experiment and the CERN accelerator teams for the outstanding performance of the LHC complex.
%
The ALICE Collaboration gratefully acknowledges the resources and support provided by all Grid centres and the Worldwide LHC Computing Grid (WLCG) collaboration.
%
The ALICE Collaboration acknowledges the following funding agencies for their support in building and running the ALICE detector:
%
A. I. Alikhanyan National Science Laboratory (Yerevan Physics Institute) Foundation (ANSL), State Committee of Science and World Federation of Scientists (WFS), Armenia;
%
Austrian Academy of Sciences, Austrian Science Fund (FWF): [M 2467-N36] and Nationalstiftung f\"{u}r Forschung, Technologie und Entwicklung, Austria;
%
Ministry of Communications and High Technologies, National Nuclear Research Center, Azerbaijan;
%
Conselho Nacional de Desenvolvimento Cient\'{\i}fico e Tecnol\'{o}gico (CNPq), Financiadora de Estudos e Projetos (Finep), Funda\c{c}\~{a}o de Amparo \`{a} Pesquisa do Estado de S\~{a}o Paulo (FAPESP) and Universidade Federal do Rio Grande do Sul (UFRGS), Brazil;
%
Ministry of Education of China (MOEC) , Ministry of Science \& Technology of China (MSTC) and National Natural Science Foundation of China (NSFC), China;
%
Ministry of Science and Education and Croatian Science Foundation, Croatia;
%
Centro de Aplicaciones Tecnol\'{o}gicas y Desarrollo Nuclear (CEADEN), Cubaenerg\'{\i}a, Cuba;
%
Ministry of Education, Youth and Sports of the Czech Republic, Czech Republic;
%
The Danish Council for Independent Research | Natural Sciences, the VILLUM FONDEN and Danish National Research Foundation (DNRF), Denmark;
%
Helsinki Institute of Physics (HIP), Finland;
%
Commissariat \`{a} l'Energie Atomique (CEA), Institut National de Physique Nucl\'{e}aire et de Physique des Particules (IN2P3) and Centre National de la Recherche Scientifique (CNRS) and R\'{e}gion des  Pays de la Loire, France;
%
Bundesministerium f\"{u}r Bildung und Forschung (BMBF) and GSI Helmholtzzentrum f\"{u}r Schwerionenforschung GmbH, Germany;
%
General Secretariat for Research and Technology, Ministry of Education, Research and Religions, Greece;
%
National Research, Development and Innovation Office, Hungary;
%
Department of Atomic Energy Government of India (DAE), Department of Science and Technology, Government of India (DST), University Grants Commission, Government of India (UGC) and Council of Scientific and Industrial Research (CSIR), India;
%
Indonesian Institute of Science, Indonesia;
%
Centro Fermi - Museo Storico della Fisica e Centro Studi e Ricerche Enrico Fermi and Istituto Nazionale di Fisica Nucleare (INFN), Italy;
%
Institute for Innovative Science and Technology , Nagasaki Institute of Applied Science (IIST), Japanese Ministry of Education, Culture, Sports, Science and Technology (MEXT) and Japan Society for the Promotion of Science (JSPS) KAKENHI, Japan;
%
Consejo Nacional de Ciencia (CONACYT) y Tecnolog\'{i}a, through Fondo de Cooperaci\'{o}n Internacional en Ciencia y Tecnolog\'{i}a (FONCICYT) and Direcci\'{o}n General de Asuntos del Personal Academico (DGAPA), Mexico;
%
Nederlandse Organisatie voor Wetenschappelijk Onderzoek (NWO), Netherlands;
%
The Research Council of Norway, Norway;
%
Commission on Science and Technology for Sustainable Development in the South (COMSATS), Pakistan;
%
Pontificia Universidad Cat\'{o}lica del Per\'{u}, Peru;
%
Ministry of Science and Higher Education and National Science Centre, Poland;
%
Korea Institute of Science and Technology Information and National Research Foundation of Korea (NRF), Republic of Korea;
%
Ministry of Education and Scientific Research, Institute of Atomic Physics and Ministry of Research and Innovation and Institute of Atomic Physics, Romania;
%
Joint Institute for Nuclear Research (JINR), Ministry of Education and Science of the Russian Federation, National Research Centre Kurchatov Institute, Russian Science Foundation and Russian Foundation for Basic Research, Russia;
%
Ministry of Education, Science, Research and Sport of the Slovak Republic, Slovakia;
%
National Research Foundation of South Africa, South Africa;
%
Swedish Research Council (VR) and Knut \& Alice Wallenberg Foundation (KAW), Sweden;
%
European Organization for Nuclear Research, Switzerland;
%
Suranaree University of Technology (SUT), National Science and Technology Development Agency (NSDTA) and Office of the Higher Education Commission under NRU project of Thailand, Thailand;
%
Turkish Atomic Energy Agency (TAEK), Turkey;
%
National Academy of  Sciences of Ukraine, Ukraine;
%
Science and Technology Facilities Council (STFC), United Kingdom;
%
National Science Foundation of the United States of America (NSF) and United States Department of Energy, Office of Nuclear Physics (DOE NP), United States of America.
